Detecting Overfitting of Deep Generative Networks via Latent Recovery

State of the art deep generative networks are capable of producing images with such incredible realism that they can be suspected of memorizing training images. It is why it is not uncommon to include visualizations of training set nearest neighbors, to suggest generated images are not simply memorized. We demonstrate this is not sufficient and motivates the need to study memorization/overfitting of deep generators with more scrutiny. This paper addresses this question by i) showing how simple losses are highly effective at reconstructing images for deep generators ii) analyzing the statistics of reconstruction errors when reconstructing training and validation images, which is the standard way to analyze overfitting in machine learning. Using this methodology, this paper shows that overfitting is not detectable in the pure GAN models proposed in the literature, in contrast with those using hybrid adversarial losses, which are amongst the most widely applied generative methods. The paper also shows that standard GAN evaluation metrics fail to capture memorization for some deep generators. Finally, the paper also shows how off-the-shelf GAN generators can be successfully applied to face inpainting and face super-resolution using the proposed reconstruction method, without hybrid adversarial losses.

==> motivations.tex <==
\subsection{Motivations} 

To begin with, while state-of-the-art generative networks yield undeniable improvement in image quality over other approaches such as patch-based methods (e.g. for inpainting~\cite{IizukaSIGGRAPH2017}), it is mostly assessed in practice by visual inspection. 
Although some recent works have been proposed to define new metrics to guide or evaluate visual performance of deep generator, such as the FID score~\cite{heusel2017gans}, inception distance \cite{salimans2016improved} or the perceptual loss \cite{johnson2016perceptual} \juju{complete this sentence ?}. 


% , typically based on nearest neighbor image matching of generated images with the dataset, and exploration of the latent space. 
Secondly, the quality of generated results have raised some suspicion (see eg \cite{arora2017gans}) \juju{autre ref ?} that deep generators might simply blending or copying verbatim features from the training dataset, like patch-based approaches in inpainting or image editing (see e.g. PatchMatch~\cite{barnes2009patchmatch}). % in computer vision applications (inpainting, texture synthesis, style transfer, etc.). 
Indeed, similarly to patch-based approaches, most deep architectures like GAN of AE are trained by explicitly trying to generate images that match the dataset distribution.
As a consequence, the images generated by state of the art GANs have such breathtaking realism, that it is tempting to think they have merely been copied from the dataset (see Figs.~\ref{fig:teaser} and \ref{fig:recovery}).
%
Such issue about memorization has been recently further supported by some studies~\cite{zhang2016understanding} that demonstrate that deep encoding neural networks are memorizing \juju{write some more about it ?}, but such memorization has yet to be proven for generators.

In practice, as illustrated in Fig.~\ref{fig:teaser}, this question is again only addressed by visual inspection. 
It is standard protocol in high fidelity GAN papers~\cite{brock2018large,karras2017progressive}, since the seminal work of \cite{goodfellow2014generative}, 
to provide a Nearest Neighbor (NN) comparison (using various metrics) between generated $G(z)$ and dataset images $y \in \cal D$ to suggest the absence of memorization. %negative. 
Notice however that, while being very popular and remarkably good to recover the pose of registered face, it is intrinsically flawed by the limitations of the metric being used.
As shown in Fig.~\ref{fig:teaser}, simply flipping a training image (while still being registered), makes it impossible to recover by NN search by any popular metric such as, Euclidean or Manhattan distance, VGG-based feature~\cite{karras2017progressive} or perceptual loss~\cite{johnson2016perceptual}.
Furthermore, the fact that latent codes interpolate reasonably well also suggests the negative. Nonetheless, both of these demonstrations remain unsatisfying. 
To the best of our knowledge, no further supporting evidence of memorization in deep generators has been demonstrated. 


%
\if0 % deplacé en contribution
\juju{move this sentence to goals /contributions ?}
Indeed, while being very popular, it has been previously noticed~\cite{metz2016unrolled} that such methodology is flawed by the limitations of the metric being used.
As shown in Fig.~\ref{fig:teaser}, simply flipping a training image (while still being registered), makes it impossible to recover by NN search by any popular metric such as VGG \cite{} or perceptual loss \cite{}.
An alternative used in this paper consists in performing the NN search in the generated image set $\mathcal G = \{G(z)\}$~\cite{metz2016unrolled} which is more robust, while using the same metric, as it can be seen in Fig.~\ref{fig:teaser}. 
\fi
%
 




Beyond these aspects of memorization and practical evaluation of generators lies the important and debated issue of privacy: % and copyright. 
How to ensure that the data used for training cannot leak by some reverse engineering, such as CNN inversion~\cite{mahendran2015understanding} or reconstruction from feature~\cite{Weinzaepfel_CVPR11} ?
%
Because GANs have seen such widespread real world application for image editing, it is imperative that we have better evaluations tools to assess how much these networks have overfit the training data. 
For example, if a user is using a neural net to inpaint faces as in \cite{li2017generative} or to perform super-resolution enhancing~\cite{dahl2017pixel}, it seems necessary to ensure verbatim copies of training images do not appear, due to privacy or even copyright concerns. 
Indeed, several  attacks against machine learning systems have been exposed in the literature \cite{papernot2016attack}.
For instance, authors in \cite{fredrikson2015inversion} designed an inversion attack to coarsely recover faces used during the training of a whitebox facial recognition neural network.
More recently, \cite{shokri2017membership} designed a membership attack allowing to determine if a given image was part of the training set of a blackbox machine learning system. 
This kind of attacks represent a serious threat to the ongoing development of machine-learning as a cloud-service. As a possible way-around, a GAN could be used to create privacy-secure version of a dataset before training a network for a particular task. Such a perspective requires to delve into the ability of GANs to keep training data private.


